Behind the Intent of Extract Method Refactoring: A Systematic Literature Review

Code refactoring is widely recognized as an essential software engineering practice to improve the understandability and maintainability of the source code. The Extract Method refactoring is considered as "Swiss army knife" of refactorings, as developers often apply it to improve their code quality. In recent years, several studies attempted to recommend Extract Method refactorings allowing the collection, analysis, and revelation of actionable data-driven insights about refactoring practices within software projects. In this paper, we aim at reviewing the current body of knowledge on existing Extract Method refactoring research and explore their limitations and potential improvement opportunities for future research efforts. Hence, researchers and practitioners begin to be aware of the state-of-the-art and identify new research opportunities in this context. We review the body of knowledge related to Extract Method refactoring in the form of a systematic literature review (SLR). After compiling an initial pool of 1,367 papers, we conducted a systematic selection and our final pool included 83 primary studies. We define three sets of research questions and systematically develop and refine a classification schema based on several criteria including their methodology, applicability, and degree of automation. The results construct a catalog of 83 Extract Method approaches indicating that several techniques have been proposed in the literature. Our results show that: (i) 38.6% of Extract Method refactoring studies primarily focus on addressing code clones; (ii) Several of the Extract Method tools incorporate the developer's involvement in the decision-making process when applying the method extraction, and (iii) the existing benchmarks are heterogeneous and do not contain the same type of information, making standardizing them for the purpose of benchmarking difficult.

==> Chart/RQ2.tex <==
\begin{figure}[t]
\centering 
\begin{tikzpicture}
\begin{scope}[scale=0.75]
\pie[rotate = 180,pos ={0,0},text=inside,outside under=38,no number]{18.3/Graphs\and18.3\%, 23.2/AST\and23.2\%, 30.5/Code\and30.5\%,9.8/Tokens\and9.8\%, 11/Metrics\and11\%, 7.3/Text\and7.3\%}
\end{scope}
\end{tikzpicture}
\caption{Percentage of \textit{Extract Method} studies, clustered by representation types.}
\label{fig:categories_clustered_rq2}
%\vspace{-.6cm}
\end{figure}

==> Tables/Metric.tex <==
\begin{table*}[!htbp]
\begin{center}
\caption{Software metrics used by the \textit{Extract Method} tools in the primary studies.}
\label{Table:Metricss_Identified_by_PSs}
\begin{adjustbox}{width=0.5\textwidth,center}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}[-3pt]{\textbf{Metrics}}   & \multicolumn{5}{c}{\textbf{Tool}} \\ 
        \cmidrule{2-6} 
      &   \textbf{AutoMed} & \textbf{SEMI} & \textbf{Unnamed2} & \textbf{LiveRef} & \textbf{AntiCopyPaster}\\ 
         \midrule
    TotalLinesOfCode & & & & & \checkmark\\
TotalSymbols & & & & & \checkmark\\
SymbolsPerLine & & & & & \checkmark\\
Area & & & & & \checkmark\\
AreaPerLine & & & & & \checkmark\\
TotalConnectivity & & & & & \checkmark\\
TotalConnectivityPerLine & & & & & \checkmark\\
FieldConnectivity & & & & & \checkmark\\
FieldConnectivityPerLine & & & & & \checkmark\\
MethodConnectivity & & & & & \checkmark\\
MethodConnectivityPerLine & & & & & \checkmark\\
MethodDeclarationLines & & & & & \checkmark\\
MethodDeclarationSymbols & & & & & \checkmark\\
MethodDeclarationSymbolsPerLine & & & & & \checkmark\\
MethodDeclarationArea & & & & & \checkmark\\
MethodDeclarationDepthPerLine & & & & & \checkmark\\
KeywordContinueTotalCount & & & & & \checkmark\\
KeywordContinueCountPerLine & & & & & \checkmark \\
KeywordForTotalCount & & & & & \checkmark\\
KeywordForCountPerLine & & & & & \checkmark\\
KeywordNewTotalCount & & & & & \checkmark\\
KeywordNewCountPerLine & & & & & \checkmark\\
KeywordSwitchTotalCount & & & & & \checkmark\\
KeywordSwitchCountPerLine & & & & & \checkmark\\
KeywordAssertTotalCount & & & & & \checkmark\\
KeywordAssertCountPerLine & & & & & \checkmark\\
KeywordSynchronizedTotalCount & & & & & \checkmark\\
KeywordSynchronizedCountPerLine & & & & & \checkmark\\
KeywordBooleanTotalCount & & & & & \checkmark\\
KeywordBooleanCountPerLine & & & & & \checkmark\\
KeywordDoTotalCount & & & & & \checkmark\\
KeywordDoCountPerLine & & & & & \checkmark\\
KeywordIfTotalCount & & & & & \checkmark\\
KeywordIfCountPerLine & & & & & \checkmark\\
KeywordThisTotalCount & & & & & \checkmark\\
KeywordThisCountPerLine & & & & & \checkmark\\
KeywordBreakTotalCount & & & & & \checkmark\\
KeywordBreakCountPerLine & & & & & \checkmark\\
KeywordDoubleTotalCount & & & & & \checkmark\\
KeywordDoubleCountPerLine & & & & & \checkmark\\
KeywordThrowTotalCount & & & & & \checkmark\\
KeywordThrowCountPerLine& & & & & \checkmark\\
KeywordByteTotalCount & & & & & \checkmark\\
KeywordByteCountPerLine & & & & & \checkmark\\
KeywordElseTotalCount & & & & & \checkmark\\
KeywordElseCountPerLine & & & & & \checkmark\\
KeywordCaseTotalCount & & & & & \checkmark\\
KeywordCaseCountPerLine & & & & & \checkmark\\
KeywordInstanceofTotalCount & & & & & \checkmark\\
KeywordInstanceofCountPerLine & & & & & \checkmark\\
KeywordReturnTotalCount & & & & & \checkmark\\
KeywordReturnCountPerLine & & & & & \checkmark\\
KeywordTransientTotalCount & & & & & \checkmark\\
KeywordTransientCountPerLine & & & & & \checkmark\\
KeywordCatchTotalCount & & & & & \checkmark\\
KeywordCatchCountPerLine & & & & & \checkmark\\
KeywordIntTotalCount & & & & & \checkmark\\
KeywordIntCountPerLine & & & & & \checkmark\\
KeywordShortTotalCount & & & & & \checkmark\\
KeywordShortCountPerLine & & & & & \checkmark\\
KeywordTryTotalCount & & & & & \checkmark\\
KeywordTryCountPerLine & & & & & \checkmark\\
KeywordCharTotalCount & & & & & \checkmark\\
KeywordCharCountPerLine & & & & & \checkmark\\
KeywordFinalTotalCount & & & & & \checkmark\\
KeywordFinalCountPerLine & & & & & \checkmark\\
KeywordFinallyTotalCount & & & & & \checkmark\\
KeywordFinallyCountPerLine & & & & & \checkmark\\
KeywordLongTotalCount & & & & & \checkmark\\
KeywordLongCountPerLine & & & & & \checkmark\\
KeywordStrictfpTotalCount & & & & & \checkmark\\
KeywordStrictfpCountPerLine & & & & & \checkmark\\
KeywordFloatTotalCount & & & & & \checkmark\\
KeywordFloatCountPerLine & & & & & \checkmark\\
KeywordSuperTotalCount & & & & & \checkmark\\
KeywordSuperCountPerLine & & & & & \checkmark\\
KeywordWhileTotalCount & & & & & \checkmark\\
KeywordWhileCountPerLine & & & & & \checkmark\\
NumberOfMethods & \checkmark & & & &  \\
NumberOfStaticMethod & \checkmark & & & & \\
MethodLinesOfCodePerMethod & \checkmark & & & & \\
LackOfCohesionOfMethod & \checkmark & \checkmark & &\checkmark & \\
WeightedMethodPerClass & \checkmark & & & & \\
McCabePerMethod & \checkmark & & & & \\
NestedBlockDepth & \checkmark & & & & \\
AfferentCoupling & \checkmark & & & & \\
NumberOfParameters & \checkmark & & & & \\
EfferentCoupling & \checkmark & & & & \\
TightClassCohesion &  &  \checkmark & & & \\
Loose Class Cohesion &  &  \checkmark & & & \\
DegreeOfCohesion-Direct &  &  \checkmark & & & \\
DegreeOfCohesion-Indirect &  &  \checkmark & & & \\
LackOfComputationalStrength &  &   & \checkmark & & \\
ParentAffinity &  &   & \checkmark & & \\
CyclomaticComplexity &  &   &  & \checkmark &\\
CognitiveComplexity &  &   &  & \checkmark &\\
Halstead &  &   &  & \checkmark &\\
MaintainabilityDegree &  &   &  & \checkmark &\\
        \bottomrule
\end{tabular} 
\end{adjustbox}
\end{center}
\end{table*}


==> Tables/name.tex <==
\begin{table*}[ht!]
  \centering
	 \caption{Related work in recommending the \textit{Extract Method} refactoring opportunities.}
	 \label{Table:Related_Work_in_Extract_Method_Refatoring}
  %\vspace{0.5cm}

\begin{adjustbox}{width=1.0\textwidth,center}
\rowcolors{2}{white}{gray!25}
\begin{tabular}{lcllllllll}\hline
\toprule
\bfseries Study & \bfseries Year  &  \bfseries Intent & \bfseries Design Property & \bfseries Representation  & \bfseries Automation (Detection)  & \bfseries Automation  (Execution) & \bfseries Semi-Automation & \bfseries Validation Method    \\
\midrule
 Lakhotia \& Deprez \cite{lakhotia1998restructuring} &  1998 &  Long Method & Semantic

 & Graphs  & Manual  & Semi-automated & Suggest Alternatives& Proof of Concept \\ %procedural \\

\textcolor{black}{Balazinska \etal \cite{balazinska1999partial}} & \textcolor{black}{1999} & \textcolor{black}{Code Clone} &  Syntactic & AST & Fully automated & Fully automated& N/A&   Proof of Concept\\

\textcolor{black}{Komondoor \& Horwitz \cite{komondoor2000semantics}} & \textcolor{black}{2000} & \textcolor{black}{Code Clone} & Semantic & Graphs  & Manual & Fully automated & N/A & Proof of Concept \\


Maruyama~\cite{maruyama2001automated} & 2001 & 
Separation of Concerns 
& Semantic & Graphs & Manual & Semi-automated & Choose Candidates &  Proof of Concept\\

\textcolor{black}{Komondoor \& Horwitz \cite{komondoor2003effective}} & \textcolor{black}{2003} & \textcolor{black}{Code Clone} &  Semantic & Graphs  & Manual  & Fully automated & N/A & Proof of Concept\\

\textcolor{black}{Ettinger \& Verbaere} \cite{ettinger2004untangling} & \textcolor{black}{2004} & \textcolor{black}{Separation of Concerns} & Semantic & Graphs & Manual  & Fully automated&  N/A&  Proof of Concept \\

 Higo \etal \cite{higo2004refactoring} &  2004 & 
 Code Clone & Textual & Source Code  & Fully automated & Semi-automated& Choose Candidates&  Case Study \\

 Higo \etal \cite{higo2004aries} &  2004  & 
 Code Clone & Semantic & Graphs & Fully automated & Fully automated & N/A& Case Study  \\

  Higo \etal \cite{higo2005aries} &  2005 & 
 Code Clone & Textual & Source Code & Fully automated & Semi-automated & Execute on Approval &  Case Study  \\

  Higo \etal \cite{higo2008metric} &   2008 & 
 Code Clone & Textual & Source Code & Fully automated & Semi automated& Execute on Approval&  Case Study \\


O'Connor \etal \cite{o2005star} & 2005 &
Separation of Concerns & Syntactic & AST & Semi-automated& Semi-automated & Suggest Alternatives &  Proof of Concept\\

\textcolor{black}{Juillerat \& Hirsbrunner} \cite{juillerat2006algorithm} & \textcolor{black}{2006} & \textcolor{black}{Code Clone} &  &  & && &  \\

\textcolor{black}{Juillerat \& Hirsbrunner} \cite{juillerat2007improving} & \textcolor{black}{2007} & \textcolor{black}{Separation of Concerns} &  &  & && &\\

 Vittek \etal \cite{vittek2007c++} &  2007 &
 Separation of Concerns
&   &   & && &  \\

Corbat \etal \cite{corbat2007ruby} & 2007 
& Separation of Concerns
& Syntactic & AST & Manual & Semi-automated & Choose Candidates  & Proof of Concept\\

 Murphy-Hill \& Black~\cite{murphy2008breaking} &  2008 &
 Separation of Concerns
&  Textual  &  Source Code & Manual  &Semi-automated & Choose Candidates  & Experiment \\ 

\textcolor{black}{Abadi \etal} \cite{abadi2008re} & \textcolor{black}{2008} &
\textcolor{black}{Separation of Concerns}
& Textual  & Source Code  & Manual & Fully automated & N/A & Case Study \\

Abadi \etal \cite{abadi2009fine} & 2009 &
Separation of Concerns
& Textual & Source Code & Manual & Fully automated & N/A&  Case Study\\

 Tsantalis \& Chatzigeorgiou~\cite{tsantalis2009identification} &  2009  &  
 Long Method &  Textual & Source Code  & Fully automated  & Semi-automated & Suggest Alternatives  & Experiment \\

 Tsantalis \& Chatzigeorgiou~\cite{tsantalis2011identification} &  2011 &
 Long Method&  Textual & Source Code  & Fully automated  & Semi-automated & Suggest Alternatives  & Experiment \\

Yang~\etal~\cite{yang2009identifying} & 2009 & Long Method
&   &  & && &  \\

\textcolor{black}{Li \& Thompson} \cite{li2009clone} & \textcolor{black}{2009} & \textcolor{black}{Code Clone} & Hybrids & AST \& Tokens & Manual & Semi-automated & Suggest Alternatives  & Case Study  \\

\textcolor{black}{Brown \& Thompson} \cite{brown2010clone} & \textcolor{black}{2010} & \textcolor{black}{Code Clone} &   Hybrids & AST \& Tokens & Manual & Semi-automated & Suggest Alternatives  & Case Study  \\

 Kanemitsu~\etal~\cite{kanemitsu2011visualization} &  2011 
&  Separation of Concerns
&    &   & &&&  \\

Meananeatra \etal \cite{meananeatra2011using} & 2011 
& Long Method
&  &  & &&  & \\


\textcolor{black}{Choi \etal} \cite{choi2011extracting}
& \textcolor{black}{2011} & Code Clone & Lexical & Tokens & Fully automated & Manual & N/A  & Case Study\\

%\textcolor{black}{Bubl{\'\i}k \& Virius}\cite{bublik2011automatic} & \textcolor{black}{2011} & \textcolor{black}{Code Clone} & \textcolor{black}{Rule-based} & \textcolor{black}{Clone pair location} & \textcolor{black}{N/A} \\

 Sharma~\cite{sharma2012identifying} &  2012 &
 Separation of Concerns & Semantic
 & Graphs  & Manual  & Fully automated & N/A  & Proof of Concept  \\

Cousot \etal \cite{cousot2012abstract} & 2012 & 
Separation of Concerns & Textual & Source Code & Manual & Fully automated & N/A &  Proof of Concept \\ 

 Tairas \& Gray \cite{tairas2012increasing} &  2012 &
 Code Clone & Syntactic 
 & AST & Fully automated  & Semi-automated & Choose Candidates &  Experiment  \\

%\textcolor{black}{Hotta \etal \cite{hotta2012identifying}} & \textcolor{black}{2012} & \textcolor{black}{Code Clone} & \textcolor{black}{Graph-based} & \textcolor{black}{Program dependency graph} & \textcolor{black}{N/A} \\

Kaya \& Fawcett \cite{kaya2013identifying} & 2013 & 
Long Method & Textual 
 & Source Code & Fully automated & Manual &N/A& Experiment \\ 

\textcolor{black}{Goto \etal \cite{goto2013extract}} & \textcolor{black}{2013} & \textcolor{black}{Code Clone} & Syntactic  & AST & Manual & Fully automated & N/A & Case Study \\

 Bian \etal \cite{bian2013spape} &  2013 
&  Code Clone
&
  Hybrids & AST \& Graphs  & Manual & Fully automated & N/A  & Experiment  \\

   Bian \etal \cite{bian2014identifying} &  2014 
&  Code Clone
&
  &   &  &&&  \\

\textcolor{black}{Krishnan \& Tsantalis} \cite{krishnan2013refactoring} & \textcolor{black}{2013} & \textcolor{black}{Code Clone} & Textual  & Source Code & Fully automated & Semi-automated & User Input  & Experiment \\

\textcolor{black}{Krishnan \& Tsantalis} \cite{krishnan2014unification} & \textcolor{black}{2014} & \textcolor{black}{Code Clone} & Hybrids  & AST \& Graphs & Fully automated & Semi-automated & User Input  & Experiment \\

\textcolor{black}{Tsantalis \etal} \cite{tsantalis2015assessing} & \textcolor{black}{2015} & \textcolor{black}{Code Clone} & Hybrids & AST \& Source Code \& Tokens &  Fully automated & Semi-automated & User Input  & Experiment \\

\textcolor{black}{Mazinanian \etal} \cite{mazinanian2016jdeodorant} & \textcolor{black}{2016} & \textcolor{black}{Code Clone} & Hybrids & AST \& Source Code \& Tokens &  Fully automated & Semi-automated & User Input &  Experiment \\

\textcolor{black}{Tsantalis \etal} \cite{tsantalis2017clone} & \textcolor{black}{2017} & \textcolor{black}{Code Clone} & Hybrids & AST \& Source Code \& Tokens &  Fully automated & Semi-automated & User Input & Experiment \\

Silva~\etal~\cite{silva2014recommending} & 2014  &
Separation of Concerns
& Textual & Source Code & Fully automated & Semi-automated & Suggest Alternatives &  Experiment  \\

Silva~\etal~\cite{silva2015jextract} & 2015 &
Separation of Concerns
&  Textual & Source Code & Fully automated & Semi-automated & Suggest Alternatives &   Experiment    \\

 Fontana \etal \cite{arcelli2015duplicated} &  2015 &
 Code Clone & Hybrids 
 & AST \& Source Code  & Fully automated & Semi-automated& Suggest Alternatives & Experiment \\ %Scenario

\textcolor{black}{Meng \etal} \cite{meng2015does} & \textcolor{black}{2015} & \textcolor{black}{Code Clone} & Syntactic & AST & Fully automated & Fully automated& N/A &  Experiment \\

\textcolor{black}{Charalampidou \etal \cite{charalampidou2015size}} & \textcolor{black}{2015} & \textcolor{black}{Long Method} & &  & && & \\

\textcolor{black}{Charalampidou \etal \cite{charalampidou2018structural}} & \textcolor{black}{2018} & \textcolor{black}{Long Method} & &  & && &\\

Charalampidou~\etal~\cite{charalampidou2016identifying} & 2016 &
Long Method &
 &  & &&& \\

 Haas \& Hummel~\cite{haas2016deriving} &  2016  & 
 Long Method &
  &   & && &  \\

   Haas \& Hummel~\cite{haas2017learning} &  2017 & 
 Long Method &
  &   & && &  \\

Xu~\etal~\cite{xu2017gems} & 2017 & 
  Separation of Concerns & Textual
 & Source Code  & Fully automated & Semi-automated & Choose Candidates &Experiment  \\

 Imazato \etal \cite{imazato2017finding} &  2017 &  Separation of Concerns &  Textual &  Source Code  & Fully automated & Manual & N/A &Experiment \\

Kaya \& Fawcett \cite{kaya2017identification} & 2017 
& Long Method
& Semantic& Graphs  & Fully automated & Fully automated & N/A & Experiment \\ 

 Maruyama \& Hayashi \cite{maruyama2017tool} &  2017 
&  Separation of Concerns
&  Textual & Source Code  & Manual & Semi-automated & Choose Candidates &  Proof of Concept \\ %Scenario

Xu \etal \cite{xu2017log} & 2017 & Long Method  & Syntactic & Metrics & Fully automated & Manual & N/A &  Experiment \\

\textcolor{black}{Chen \etal} \cite{chen2017tool} & \textcolor{black}{2017} & \textcolor{black}{Code Clone} &  Syntactic  & AST & Manual & Fully automated & N/A & Case Study\\

\textcolor{black}{Ettinger \& Tyszberowicz} \cite{ettinger2016duplication} & \textcolor{black}{2016} & \textcolor{black}{Code Clone} & Textual  & Source Code &  Manual & Fully automated & N/A &Proof of Concept \\

\textcolor{black}{Ettinger \etal} \cite{ettinger2017efficient} & \textcolor{black}{2017} & \textcolor{black}{Code Clone} & Semantic & Graphs & Manual & Fully automated &N/A  & Proof of Concept \\

 Meananeatra \etal \cite{meananeatra2018refactoring} &  2018 
&  Long Method
&  Hybrids & AST \& Graphs & Manual& Semi-automated & Execute on Approval &  Case Study  \\

Choi \etal \cite{choi2018investigation} & 2018 
& Long Method
& Syntactic & Metrics & Fully automated & Manual & N/A &  Experiment \\



 Yue~\etal~\cite{yue2018automatic} &  2018 
&   Code Clone & Syntactic 
  &  AST  & Fully automated  & Manual & N/A &  Experiment \\

\textcolor{black}{Vidal \etal} \cite{vidal2018assessing} & \textcolor{black}{2018} & \textcolor{black}{Long Method} & Textual  & Source Code & Fully automated& Semi-automated & Choose Candidates &Case Study\\

Yoshida~\etal~\cite{yoshida2019proactive} & 2019 
& Code Clone
& Hybrids & AST \& Tokens & Fully automated & Semi-automated & Choose Candidates &  Experiment \\

\textcolor{black}{Shin \cite{shin2019study}} & \textcolor{black}{2019} & \textcolor{black}{Code Clone} &  &  & && & \\

\textcolor{black}{Barrs \& Oprescu \cite{baars2019towards}} & \textcolor{black}{2019} & \textcolor{black}{Code Clone} &  Hybrids & AST \& Graphs & Fully automated & Manual & N/A & Experiment \\


 Antezana \cite{antezana2019toad} &  2019  & 
 Long Method & Textual
 &  Source Code  & Manual & Semi-automated & Choose Candidates & Experiment  \\

 Alcocer \etal \cite{alcocer2020improving} &  2020 & 
 Long Method & Textual
 &  Source Code  & Manual & Semi-automated & Choose Candidates &  Experiment  \\

Nyamawe \etal \cite{nyamawe2019automated} & 2019 
& Separation of Concerns
&  Textual & Text   & Fully automated & Manual & N/A &  Experiment \\

Nyamawe \etal \cite{nyamawe2020feature} & 2020 
& Separation of Concerns
&  Textual & Text   & Fully automated & Manual & N/A &  Experiment \\

 Krasniqi \& Cleland-Huang \cite{krasniqi2020enhancing} &  2020 &  
 Separation of Concerns &
 Textual & Text   & Fully automated & Manual & N/A &   Experiment \\

Abid \etal \cite{abid2020does} & 2020 
& Separation of Concerns
&  &  & && & \\

 Sheneamer  \cite{sheneamer2020automatic} &  2020 &  Code Clone
&  Hybrids &  AST \& Graphs \& Tokens   & Fully automated  & Manual & Choose Candidates&  Experiment \\

Aniche~\etal~\cite{aniche2020effectiveness} & 2020 
& Separation of Concerns
&  Syntactic &  Metrics  & Fully automated & Manual & N/A&  Experiment \\

 Van~der~Leij~\etal~\cite{van2021data} &  2021 &  
 Separation of Concerns &
Syntactic &  Metrics  & Fully automated & Manual & N/A&  Experiment \\

Sagar \etal \cite{sagar2021comparing} & 2021 &
Separation of Concerns & Hybrids
 & Text \& Metrics  & Fully automated & Manual & N/A &  Experiment  \\

 AlOmar \etal \cite{alomar2022documentation} &  2022 & 
 Separation of Concerns & Textual &  Text  & Fully automated & Manual & N/A&  Experiment \\

Nyamawe \cite{nyamawe2022mining} & 2022 
& Separation of Concerns &
Textual &  Text  & Fully automated & Manual & N/A& Experiment \\

 Shahidi~\etal~\cite{shahidi2022automated} &  2022 &  
 Long Method &
  &    & && & \\

Tiwari \&  Joshi~\cite{tiwari2022identifying} & 2022 & Long Method & Semantic & Graphs  & Fully automated & Manual & N/A&  Experiment \\

 Fernandes \etal \cite{fernandes2022liveref} &  2022 &  Long Method  
& Syntactic  &  Metrics & Fully automated& Semi-automated & Execute on Approval&   Experiment  \\

 Fernandes \etal \cite{fernandes2022live} &  2022 &  Long Method  
& Syntactic  &  Metrics & Fully automated& Semi-automated & Execute on Approval&  Experiment \\

AlOmar \etal \cite{alomar2022anticopypaster} & 2022 & Code Clone 
& Syntactic  &  Metrics & Fully automated& Semi-automated & Execute on Approval&  Experiment \\

AlOmar \etal \cite{alomar2023just} &  2023 & Code Clone 
&  Syntactic  &  Metrics & Fully automated& Semi-automated & Execute on Approval&  Experiment \\

 Cui \etal \cite{cui2023rems} &  2023 &
 Separation of Concerns
& Semantic  &   Graphs & Fully automated & Manual& N/A & Experiment \\

\textcolor{black}{Thy \etal \cite{thy15adventure}} & \textcolor{black}{2023} & \textcolor{black}{Separation of Concerns} & Textual & Source Code &  Fullu automated& Fully automated & N/A &  Case Study \\

\textcolor{black}{Palit \etal \cite{palit14automatic}} & \textcolor{black}{2023} & \textcolor{black}{Separation of Concerns} &  Semantic&  Graphs & Fully automated  & Manual& N/A  & Experiment\\

\bottomrule
\end{tabular}
\end{adjustbox}

\vspace{-.3cm}
\end{table*}
